Massive Dimensions Reduction and Hybridization with Meta-heuristics in Deep Learning

Deep learning is mainly based on utilizing gradient-based optimization for training Deep Neural Network (DNN) models. Although robust and widely used, gradient-based optimization algorithms are prone to getting stuck in local minima. In this modern deep learning era, the state-of-the-art DNN models have millions and billions of parameters, including weights and biases, making them huge-scale optimization problems in terms of search space. Tuning a huge number of parameters is a challenging task that causes vanishing/exploding gradients and overfitting; likewise, utilized loss functions do not exactly represent our targeted performance metrics. A practical solution to exploring large and complex solution space is meta-heuristic algorithms. Since DNNs exceed thousands and millions of parameters, even robust meta-heuristic algorithms, such as Differential Evolution, struggle to efficiently explore and converge in such huge-dimensional search spaces, leading to very slow convergence and high memory demand. To tackle the mentioned curse of dimensionality, the concept of blocking was recently proposed as a technique that reduces the search space dimensions by grouping them into blocks. In this study, we aim to introduce Histogram-based Blocking Differential Evolution (HBDE), a novel approach that hybridizes gradient-based and gradient-free algorithms to optimize parameters. Experimental results demonstrated that the HBDE could reduce the parameters in the ResNet-18 model from 11M to 3K during the training/optimizing phase by metaheuristics, namely, the proposed HBDE, which outperforms baseline gradient-based and parent gradient-free DE algorithms evaluated on CIFAR-10 and CIFAR-100 datasets showcasing its effectiveness with reduced computational demands for the very first time.

==> old_cifar10.tex <==
\begin{table}
    \centering
    \caption{Results of training ResNet-18 model evaluated on CIFAR10 based on the f1-score metric. The size of parameters in the search space is indicated as $D$.}
\begin{tabular}{l|lll}
\hline
Algorithm  & Size ($D$)    & Train   & Test    \\ \hline
Adam       & 11M  & 97.23 & 80.77 \\ \hline
Classic DE & 11M  & 99.24 & 81.55 \\
 BDE       & 3.4K & \textbf{99.34} & \textbf{82.00} \\
BORVDE     & 3.4K & \textbf{99.30} & \textbf{81.79} \\ \hline
\end{tabular}
    
    \label{tab:cifar10}
\end{table}

==> old_cifar100.tex <==
\begin{table}
    \centering
    \caption{Results of training ResNet-18 model evaluated on CIFAR100 based on the f1-score metric. The size of parameters in the search space is indicated as $D$.}
\begin{tabular}{l|lll}
\hline
Algorithm  & Size ($D$)      & Train   & Test    \\ \hline
Adam       & $11$M  & 90.76 & 52.61 \\ \hline
Classic DE & $11$M  & 92.60 & 53.41\\
 BDE       & $3.5$K   & \textbf{93.19} & \textbf{53.22} \\
BORVDE     & $3.5$K & \textbf{92.91} & \textbf{53.20} \\ \hline
\end{tabular}
    
    \label{tab:cifar100}
\end{table}
